TrustBoost: Boosting Trust among Interoperable Blockchains

Currently there exist many blockchains with weak trust guarantees, limiting applications and participation. Existing solutions to boost the trust using a stronger blockchain, e.g., via checkpointing, requires the weaker blockchain to give up sovereignty. In this paper, we propose a family of protocols in which multiple blockchains interact to create a combined ledger with boosted trust. We show that even if several of the interacting blockchains cease to provide security guarantees, the combined ledger continues to be secure - our TrustBoost protocols achieve the optimal threshold of tolerating the insecure blockchains. This optimality, along with the necessity of blockchain interactions, is formally shown within the classic shared memory model, tackling the long standing open challenge of solving consensus in the presence of both Byzantine objects and processes. Furthermore, our proposed construction of TrustBoost simply operates via smart contracts and require no change to the underlying consensus protocols of the participating blockchains, a form of ``consensus on top of consensus''. The protocols are lightweight and can be used on specific (e.g., high value) transactions; we demonstrate the practicality by implementing and deploying TrustBoost as cross-chain smart contracts in the Cosmos ecosystem using approximately 3,000 lines of Rust code, made available as open source. Our evaluation shows that using 10 Cosmos chains in a local testnet, TrustBoost has a gas cost of roughly $2 with a latency of 2 minutes per request, which is in line with the cost on a high security chain such as Bitcoin or Ethereum

==> 2_model.tex <==
\section{Preliminaries}

Since our goal is to achieve consensus on top of consensus (i.e., blockchains), it is natural to model blockchains as \textit{validators} in the ``meta'' consensus protocol, and blockchain users as  \textit{clients} that can query states of blockchains via RPCs. Hence, we have the following participation and network model.

\subsection{Model}

\noindent {\bf Participants.} 
In this paper, the distributed protocols involve two types of participants: (i) validators, and (ii) clients. We assume Byzantine faults that can behave arbitrarily. Let $m$ be the number of validators and  $f$ be the number of Byzantine validators. We assume no trust from the clients, i.e., we allow any number of Byzantine clients, but only honest clients enjoy the guarantees of the protocol. %We assume participants are connected with authenticated channels like in~\cite{lamport1982byzantine}. In addition, we assume the existence of a public-key infrastructure (PKI) for the set of validators, i.e., the public keys of all validators are known to all validators and clients. However, the PKI may or may not be needed by the distributed protocol; and in the case that it is indeed used, the authenticated channel assumption is unnecessary. 
We suppose one of the following two prerequisites is met:  (1) all participants are connected via authenticated channels (see \cite{lamport1982byzantine}); (2) there exists a public-key infrastructure (PKI) for the set of validators, i.e., the public keys of all validators are known to all validators and clients.

\noindent {\bf Network model.} %The communication network between validators is represented by an undirected graph $G = (V_G,E_G)$. Validators $i$ and $j$ can send messages to each other if and only if they are adjacent in $G$, i.e., $(i,j) \in E_G$. A path $P$ in an graph $G = (V_G,E_G)$ is a finite sequence of edges which joins a sequence of distinct vertices. An graph $G$ is called connected if there is a path between every node pair in $G$; An graph $G$ is called $k$-connected if $G$ is connected after removing $k-1$ arbitrary nodes. 
Validators are in a fully connected network among themselves. We say the validators are in a \textit{passive mode} if they do not communicate with each other; otherwise they are in  an \textit{active mode}. 
Each client is also connected to all the validators -- clients only receive messages from the validators, but do not transmit any messages to the validators. Note that allowing bidirectional communications between validators and clients would turn the passive mode into the active mode as clients can help forward messages. %All clients are also in a fully connected network so that they can possibly sync up state with each other or bootstrap new clients. %\xw{Relaxing this weird assumption: for consensus, there is no communication among clients; for ledger consensus, clients communicate only for proving the confirmation of certain transactions (e.g., the sender proves to the receiver that the transaction input has been confirmed, and this communication can be synchronous and out-of-band.} 
We assume the network is partially synchronous, i.e., there is a global stabilization time ($GST$) chosen by the adversary, unknown to the honest parties and also to the protocol designer, such that after $GST$, all messages sent between honest parties are delivered within $\Delta$ time. Before $GST$, the adversary can delay messages arbitrarily.  When $GST=0$, the network becomes synchronous.


%Validators work together to decide a total ordering of all transactions submitted by clients. Each client initially starts with the same state and updates the state by executing all transactions in its TrustBoost ledger. 

%Normally in a distributed ledger, the state is maintained/updated by validators. However, in Section~\ref{sec:protocol} we will see that each validator in TrustBoost is implemented by an existing programmable blockchain. And we would like to have ``stateless validators'' as it could be costly to store the data/state on-chain. Therefore, the task of state updating is designated to clients in TrustBoost. 

%\noindent {Transactions and Ledger}. Clients generate transactions. They communicate these transactions to the validators (see network model below).  and maintain a log of transactions (called TrustBoost ledger) locally. 





%We point out that the robust ledger combiner fits perfectly in our model, where the ledgers are validators and the observers are clients in our notion. In Section~\ref{sec:converse}, we formally show that what robust ledger combiner tried to do is actually impossible if the ledgers cannot ``communicate'' with each other.

%\noindent {\bf Network.} We assume the network is partial synchronous. There is a global stabilization time (GST) chosen by the adversary, unknown to the honest parties and also to the protocol designer. Before GST, the adversary can delay messages arbitrarily. After GST, all messages sent between honest parties are delivered within $\Delta$ time.

%\noindent {\bf Graph connectivity.} A path $P$ in an graph $G = (V_G,E_G)$ is a finite sequence of edges which joins a sequence of distinct vertices. An graph $G$ is called connected if there is a path between every node pair in $G$; An graph $G$ is called $k$-connected if $G$ is connected after removing $k-1$ arbitrary nodes. 

\subsection{Distributed protocols}
{\color{red} \textbf{TODO: change definitions according to reviews.}}

To study the security guarantee of the ``meta'' consensus protocol, we define the following client consensus problems. 

% \pv{need to point out that consensus is on top of blockchains and hence below is the right model for such "meta" consensus}
\noindent {\bf Client consensus.} We start with the problem of (binary) \textit{client consensus} %(as defined in Definition~\ref{def:consensus}), 
where each validator starts with some initial value (0 or 1) and all (honest) clients try to commit the same value by the end of the protocol. %And we can see that the problem of ledger consensus is just a multi-shot version of consensus. \xw{Is there a simple reduction from SMR to consensus?}
\begin{defn}[Client Consensus]
\label{def:consensus}
\hfill
\begin{itemize}
    % \item \textbf{Agreement}: If some honest client commits a value, every honest client will commit the same value. 
    \item \textbf{Agreement}: No conflicting values are committed by honest clients.
    \item \textbf{Validity}: If every honest validator starts with the same value, this value will be committed by honest clients.
    \item \textbf{Termination}: Every honest client commits one of the values. %If messages are delivered quickly, the consensus protocol terminates quickly.
\end{itemize}
\end{defn}


We are also interested in a relaxed notion of client consensus, called \textit{ABC client consensus}, derived from~\cite{sliwinski2019abc}. The key insight leading to this relaxation is that Byzantine parties do not need to enjoy any guarantees. %In this paper, we show that to achieve ABC client consensus (as defined in Definition~\ref{def:abc}), no communication among validators will be needed.

\begin{defn}[ABC Client Consensus]
\label{def:abc}
\hfill
\begin{itemize}
    % \item \textbf{Agreement}: If some honest client commits a value, every honest client will commit the same value. 
    \item \textbf{Agreement}: Same as in Definition~\ref{def:consensus}. %No conflicting values are committed by honest clients.
    \item \textbf{Validity}: Same as in Definition~\ref{def:consensus}. %If every honest validator starts with the same value, this value will be committed by honest clients.
    \item \textbf{Honest termination}: If every honest validator starts with the same value, this value will be committed by honest clients. % If messages are delivered quickly, the ABC consensus protocol terminates quickly.
\end{itemize}
\end{defn}

\noindent {\bf Contrast with traditional consensus protocols.} In the traditional (ABC) consensus problem~\cite{dolev1983authenticated,sliwinski2019abc}, there is no client and the guarantees are enjoyed by the validators. It is not hard to see that any traditional (ABC) consensus protocol can be used to solve (ABC) client consensus in our setting: Let $3f+1$ validators run the traditional (ABC) consensus consensus protocol and send the committed value to all clients; each client commits the majority value received from those $3f+1$ validators (note that solving both consensus and ABC consensus would need $m>3f$ in partial synchrony). Therefore, any impossibility result (necessary condition) for the problem of (ABC) client consensus consensus in our model also applies to traditional (ABC) consensus. On the other hand, solving the problem of client (ABC) consensus in our model does not necessarily solve traditional (ABC) consensus. Indeed, in the above example, the other $m-3f-1$ validators do not even participate in the protocol so that they cannot commit any value. In \S\ref{sec:converse}, we will also see that ABC consensus can be solved in our model without any communication among validators. However, this is not possible in the traditional model because, without communication, basically nothing can be done in a distributed system.

\noindent {\bf Ledger consensus.} %It is known that consensus protocols can be used to solve the problem of \textit{ledger consensus}, i.e., \textit{state machine replication (SMR)}~\cite{smr}. In our model, we also slightly modify the definition of ledger consensus such that it now requires all clients maintain a list of transactions that grows in length, called a \textit{public ledger} (cf. Definition~\ref{def:pl}), with the help of the validators. Validators participate in the protocol to decide a total ordering of all transactions. Each client initially starts with the same state and updates the state by executing all transactions in its ledger. The definition of ledger consensus in our model and a comparison with the traditional definition can be found in Appendix~\ref{app:def}.
It is known that consensus protocols can be used to solve the problem of \textit{ledger consensus}, i.e., \textit{state machine replication (SMR)}~\cite{smr}. In our model, we also slightly modify the definition of ledger consensus such that it now requires all clients to maintain a list of transactions that grows in length, called a \textit{public ledger} (cf. Definition~\ref{def:pl}), with the help of the validators. Validators participate in the protocol to decide a total ordering of all transactions. Each client initially starts with the same state and updates the state by executing all transactions in its ledger. %The definition of ledger consensus in our model and a comparison with the traditional definition can be found in Appendix~\ref{app:def}.
We first define the notion of a public ledger.
\begin{defn}[Public ledger]
\label{def:pl}
A ledger $\mathcal{L}$ is a growing list of transactions that provides the following two client interfaces:
\begin{itemize}
    \item Submit: a client can submit a transaction $tx$ to $\mathcal{L}$ by calling {\sf submit}$(tx)$.
    \item Check: a client can check whether $tx \in \mathcal{L}$ by calling {\sf check}$(tx)$. If {\sf check}$(tx)$ returns true, the client will commit $tx$.
\end{itemize}

\end{defn}

In the problem of client ledger consensus, we allow the following synchronous out-of-band communications among clients: 1) clients can send transactions to validators, but still clients send no other message to validators; 2) clients can communicate with each other only to prove the confirmation of certain transactions (i.e., allowed to sync up state with each other or bootstrap new clients).
%Transactions are input to the validators by the environment $\mathcal{Z}$. 
The guarantees of client ledger consensus are defined as follows.
% \begin{defn}[Client ledger consensus]
% \label{def:ledger}
% \hfill
% \begin{itemize}
%     \item \textbf{Safety}: . If $[tx_0, tx_1, \cdots, tx_i]$ and $[tx_0', tx_1', \cdots, tx_{i'}']$ are two ledgers output by two honest clients, then $tx_j = tx_j'$ for all $j \leq \min(i,i')$.
%     \item \textbf{Liveness}: If a transaction $tx$ is input to at least one honest validator, then every honest clients eventually outputs a ledger containing $tx$.
% \end{itemize}
% \end{defn}

\begin{defn}[Client ledger consensus]
\label{def:ledger}
\hfill
\begin{itemize}
    \item \textbf{Agreement}: If some honest client commits $tx$, every honest client will also commit $tx$; moreover, $tx$ appears at the same place in the ledgers of all honest clients. Equivalently, if $[tx_0, tx_1, \cdots, tx_i]$ and $[tx_0', tx_1', \cdots, tx_{i'}']$ are two ledgers output by two honest clients, then $tx_j = tx_j'$ for all $j \leq \min(i,i')$.
    % \item \textbf{Validity}: If a client submits $tx$ to all honest validators, $tx$ will be committed by all honest clients.
    \item \textbf{Termination}: If a client submits $tx$ to all honest validators, $tx$ will be committed by all honest clients. % If messages are delivered quickly, $tx$ will be committed quickly.
\end{itemize}
\end{defn}

%We can see that the problem of ledger consensus is just a multi-shot version of consensus. \xw{Is there a simple reduction from SMR to consensus?} In addition, since a ledger consensus protocol services any number of clients, it needs to provide public verifiability. Following the definition in~\cite{momose2021multi}, there is a predefined Boolean function $\mathsf{Verify}$; a client outputs a log of transactions $\mathsf{log} = [tx_0, tx_1, \cdots, tx_i]$ if and only if there exists a proof $\pi$ such that $\mathsf{Verify}(\mathsf{log}, \pi) = 1$ and there do not exist $\pi'$ and $\mathsf{log}'$ such that $\mathsf{log}$ and $\mathsf{log}'$ violate safety and $\mathsf{Verify}(\mathsf{log}', \pi') = 1$. A typical way to achieve it is to have clients collect signatures on the $\mathsf{log}$ from $m-f$ validators, which serve as a publicly verifiable proof for the $\mathsf{log}$, usually also called a quorum certificate.

Similarly, ABC consensus can also be used to build a public ledger, although without total ordering of the transactions. However, this suffices to implement the functionality of a cryptocurrency like {\sf Bitcoin} as shown in~\cite{sliwinski2019abc,baudet2020fastpay,guerraoui2019consensus}. Suppose the transaction space is now equipped with a conflict relation (e.g. double spend transactions in {\sf Bitcoin}), then the problem of ABC client ledger consensus is defined as follows.

\begin{defn}[ABC client ledger consensus]
\label{def:abc_ledger}
\hfill
\begin{itemize}
    \item \textbf{Weak agreement}: If some honest client commits $tx$, every honest client will also commit $tx$. 
    % \item \textbf{Validity}: If every honest validator observes the same transaction (there are no conflicting transactions), this transaction will be committed by honest clients.
    \item \textbf{Honest termination}: If a client submits $tx$ to all honest validators and there are no conflicting transactions, $tx$ will be committed by all honest clients.% If messages are delivered quickly, $tx$ will be committed quickly.
\end{itemize}
\end{defn}

%We can also define public verifiability for ABC ledger consensus. Namely, there is a predefined Boolean function $\mathsf{Verify}$; a client commits a transactions $tx$ if and only if there exists a proof $\pi$ such that $\mathsf{Verify}(tx, \pi) = 1$ and there do not exist $\pi'$ and $tx'$ such that $tx'$ conflicts $tx$ and $\mathsf{Verify}(tx', \pi') = 1$.

%\noindent {\bf Contrast with traditional ledger consensus protocols.} In the problem of traditional (ABC) ledger consensus~\cite{yin2019hotstuff,sliwinski2019abc}, the state is maintained/updated by validators instead of clients. In \S\ref{sec:protocol}, we will see that each validator in our protocol called \tb is implemented by an existing programmable blockchain. And we would like to have ``stateless validators'' as it could be costly to store the data/state on the blockchains. Therefore, the task of state updating is designated to clients in our model.
% \peiyao{Why do we say blockchain validators are stateless? Do they still maintain local states (which global states are derived from)?} \xw{We'd like to have, but we don't. I removed this.}
It is not hard to see that any traditional (ABC) ledger consensus protocol can be used to solve (ABC) client ledger consensus in our model: the validators just run a traditional (ABC) ledger consensus protocol and send the committed ledgers to the clients. This allows us to construct \tb in a black-box manner. On the other hand, similar to ABC client consensus, ABC client ledger consensus can be solved without any communication among the validators. This observation leads to the protocol \tblite in \S\ref{sec:lite}, where no CCC is needed.





==> app_definition.tex <==
\section{Definitions of Ledger Consensus}
\label{app:def}

It is known that consensus protocols can be used to solve the problem of \textit{ledger consensus}, i.e., \textit{state machine replication (SMR)}~\cite{smr}. In our model, we also slightly modify the definition of ledger consensus such that it now requires all clients to maintain a list of transactions that grows in length, called a \textit{public ledger} (cf. Definition~\ref{def:pl}), with the help of the validators. Validators participate in the protocol to decide a total ordering of all transactions. Each client initially starts with the same state and updates the state by executing all transactions in its ledger. %The definition of ledger consensus in our model and a comparison with the traditional definition can be found in Appendix~\ref{app:def}.
We first define the notion of a public ledger.
\begin{defn}[Public ledger]
\label{def:pl}
A ledger $\mathcal{L}$ is a growing list of transactions that provides the following two client interfaces:
\begin{itemize}
    \item Submit: a client can submit a transaction $tx$ to $\mathcal{L}$ by calling {\sf submit}$(tx)$.
    \item Check: a client can check whether $tx \in \mathcal{L}$ by calling {\sf check}$(tx)$. If {\sf check}$(tx)$ returns true, the client will commit $tx$.
\end{itemize}

\end{defn}

In the problem of client ledger consensus, we allow the following synchronous out-of-band communications among clients: 1) clients can send transactions to validators, but still clients send no other message to validators; 2) clients can communicate with each other only to prove the confirmation of certain transactions (i.e., allowed to sync up state with each other or bootstrap new clients).
%Transactions are input to the validators by the environment $\mathcal{Z}$. 
The guarantees of client ledger consensus are defined as follows.
% \begin{defn}[Client ledger consensus]
% \label{def:ledger}
% \hfill
% \begin{itemize}
%     \item \textbf{Safety}: . If $[tx_0, tx_1, \cdots, tx_i]$ and $[tx_0', tx_1', \cdots, tx_{i'}']$ are two ledgers output by two honest clients, then $tx_j = tx_j'$ for all $j \leq \min(i,i')$.
%     \item \textbf{Liveness}: If a transaction $tx$ is input to at least one honest validator, then every honest clients eventually outputs a ledger containing $tx$.
% \end{itemize}
% \end{defn}

\begin{defn}[Client ledger consensus]
\label{def:ledger}
\hfill
\begin{itemize}
    \item \textbf{Agreement}: If some honest client commits $tx$, every honest client will also commit $tx$; moreover, $tx$ appears at the same place in the ledgers of all honest clients. Equivalently, if $[tx_0, tx_1, \cdots, tx_i]$ and $[tx_0', tx_1', \cdots, tx_{i'}']$ are two ledgers output by two honest clients, then $tx_j = tx_j'$ for all $j \leq \min(i,i')$.
    % \item \textbf{Validity}: If a client submits $tx$ to all honest validators, $tx$ will be committed by all honest clients.
    \item \textbf{Termination}: If a client submits $tx$ to all honest validators, $tx$ will be committed by all honest clients. If messages are delivered quickly, $tx$ will be committed quickly.
\end{itemize}
\end{defn}

%We can see that the problem of ledger consensus is just a multi-shot version of consensus. \xw{Is there a simple reduction from SMR to consensus?} In addition, since a ledger consensus protocol services any number of clients, it needs to provide public verifiability. Following the definition in~\cite{momose2021multi}, there is a predefined Boolean function $\mathsf{Verify}$; a client outputs a log of transactions $\mathsf{log} = [tx_0, tx_1, \cdots, tx_i]$ if and only if there exists a proof $\pi$ such that $\mathsf{Verify}(\mathsf{log}, \pi) = 1$ and there do not exist $\pi'$ and $\mathsf{log}'$ such that $\mathsf{log}$ and $\mathsf{log}'$ violate safety and $\mathsf{Verify}(\mathsf{log}', \pi') = 1$. A typical way to achieve it is to have clients collect signatures on the $\mathsf{log}$ from $m-f$ validators, which serve as a publicly verifiable proof for the $\mathsf{log}$, usually also called a quorum certificate.

Similarly, ABC can also be used to build a public ledger, although without total ordering of the transactions. However, this suffices to implement the functionality of a cryptocurrency like {\sf Bitcoin} as shown in~\cite{sliwinski2019abc,baudet2020fastpay,guerraoui2019consensus}. Suppose the transaction space is now equipped with a conflict relation (e.g. double spend transactions in {\sf Bitcoin}), then the problem of ABC client ledger consensus is defined as follows.

\begin{defn}[ABC client ledger consensus]
\label{def:abc_ledger}
\hfill
\begin{itemize}
    \item \textbf{Weak agreement}: If some honest client commits $tx$, every honest client will also commit $tx$. 
    % \item \textbf{Validity}: If every honest validator observes the same transaction (there are no conflicting transactions), this transaction will be committed by honest clients.
    \item \textbf{Honest termination}: If a client submits $tx$ to all honest validators and there are no conflicting transactions, $tx$ will be committed by all honest clients. If messages are delivered quickly, $tx$ will be committed quickly.
\end{itemize}
\end{defn}

%We can also define public verifiability for ABC ledger consensus. Namely, there is a predefined Boolean function $\mathsf{Verify}$; a client commits a transactions $tx$ if and only if there exists a proof $\pi$ such that $\mathsf{Verify}(tx, \pi) = 1$ and there do not exist $\pi'$ and $tx'$ such that $tx'$ conflicts $tx$ and $\mathsf{Verify}(tx', \pi') = 1$.

%\noindent {\bf Contrast with traditional ledger consensus protocols.} In the problem of traditional (ABC) ledger consensus~\cite{yin2019hotstuff,sliwinski2019abc}, the state is maintained/updated by validators instead of clients. In \S\ref{sec:protocol}, we will see that each validator in our protocol called \tb is implemented by an existing programmable blockchain. And we would like to have ``stateless validators'' as it could be costly to store the data/state on the blockchains. Therefore, the task of state updating is designated to clients in our model.
% \peiyao{Why do we say blockchain validators are stateless? Do they still maintain local states (which global states are derived from)?} \xw{We'd like to have, but we don't. I removed this.}
It is not hard to see that any traditional (ABC) ledger consensus protocol can be used to solve (ABC) client ledger consensus in our model: the validators just run a traditional (ABC) ledger consensus protocol and send the committed ledgers to the clients. This allows us to construct \tb in a black-box manner. On the other hand, similar to ABC client consensus, ABC client ledger consensus can be solved without any communication among the validators. This observation leads to the protocol \tblite in \S\ref{sec:lite}, where no CCC is needed.

% \peiyao{What's the benefit of defining client consensus? it looks like an application-motivated definition} \xw{To sharply argue IBC is necessary for consensus, but not for ABC.}

==> app_proof.tex <==
\section{Proof of Theorem~\ref{thm:passive}}
\label{app:proof1}

\begin{proof}
Since in our model, the distributed protocols may or may not use PKI, we prove the strongest results: for the negative results (i.e., ``only if'' parts), we assume PKI is used; and for the positive results (i.e., ``if'' parts), we avoid using PKI.

\hfill

\noindent (1) Client consensus:

\noindent \textit{Only if}: 
Seeking a contradiction, let us assume there is a protocol that solves client consensus in passive mode. Divide all the clients into two sets: $X$ and $Y$ each with at least one honest client. We first construct the following $m+1$ worlds. See Fig.~\ref{fig:converse2}.

\begin{figure*}
    \centering
    \includegraphics[width=0.85\textwidth]{figures/worlds.pdf}
    \caption{Different worlds in the proof of Theorem~\ref{thm:passive}.}
    \label{fig:converse2}
    % \vspace{-0.6cm}
\end{figure*}

\noindent {\bf World $1.i$ ($0\leq i \leq m$):} In world $1.i$, the first $i$ validators start with value 0 and the rest $m-i$ validators start with value 1. By termination, in all $m+1$ worlds, clients in $X$ and $Y$ must eventually commit some value. By validity, the committed value must be 1 in world $1.0$ and 0 in world $1.m$.%\peiyao{why? in world 1.1 only the first validator starts with value 0.}\xw{Fixed.} 
Then there must exist some integer $0\leq j\leq m-1$ such that the committed value is 1 in world $1.j$ and 0 in world $1.(j+1)$. 
Now consider  the following world:

%\noindent {\bf World $2.j$:} In world $2.j$, the first $j$ validators start with value 0 and the rest $m-j$ validators start with value 1. Clients in $X$ have crashed. By termination, clients in $Y$ must eventually commit some value. 

%\noindent {\bf World $2.(j+1)$:} In world $2.(j+1)$, the first $j+1$ validators start with value 0 and the rest $m-j-1$ validators start with value 1. Clients in $X$ have crashed. By termination, clients in $Y$ must eventually commit some value. 

%Next, the problem can be divided into three cases:

%\noindent \textit{Case 1.} Clients in $Y$ commit 0 in world $2.j$. Then we consider the following world.
    
%\noindent {\bf World $3$:} In world $3$, the first $j$ validators start with value 0 and the rest $m-j$ validators start with value 1. The messages between $X$ and $Y$ are delayed by the adversary. However, the view of $X$ in this world will be indistinguishable to the view of $X$ in world $1.j$ and the view of $Y$ in this world will be indistinguishable to the view of $Y$ to world $2.j$. Therefore, $X$ will commit 1 and $Y$ will commit 0. This violates the agreement property.

%\noindent \textit{Case 2.} Clients in $Y$ commit 1 in world $2.(j+1)$. This case can be contracted in the same way as case 1.

%\noindent \textit{Case 3.} Clients in $Y$ commit 1 in world $2.j$ and clients in $Y$ commit 0 in world $2.(j+1)$. Then we consider the following world.
    
\noindent {\bf World $2$:} World $2$ will be a hybrid world where the view of clients in $X$ in this world will be indistinguishable to their views in world $1.(j+1)$ and the view of clients in $Y$ in this world will be indistinguishable to their view in world $1.j$. In world $2$, the first $j$ validators start with value 0 and the last $m-j-1$ validators start with value 1. The adversary will use its Byzantine power to corrupt the $(j+1)$-th validator to perform a split-brain attack and make $X$ and $Y$ each believe that they are in their respective worlds. The $(j+1)$-th validator will equivocate and act as if its starting value is 0 when communicating with $X$ and as if its 1 when communicating with $Y$.
And since there is no communication among the validators, their views will be indistinguishable to the views in worlds $1.j$ and $1.(j+1)$. Moreover, the view of $X$ in this world will be indistinguishable to the view of $X$ in world $1.(j+1)$ and the view of $Y$ in this world will be indistinguishable to the view of $Y$ to world $1.j$. Therefore, $X$ will commit 0 and $Y$ will commit 1. This violates the agreement property.

\hfill

\noindent \textit{If}: With $f=0$, we solve the problem of client consensus in the passive mode. The protocol is simple: the validators just send their values to all clients; and the client commits a value if it receives the same value from all $m$ validators; otherwise if the client receives both 0 and 1, it commits 0 by default. It is easy to check that this protocol satisfies agreement, validity and termination; Moreover, there is no communication among the validators.

\hfill

\noindent (2) ABC client consensus:

\noindent \textit{Only if}: Seeking a contradiction, let us assume there is a protocol that claims to solve ABC client consensus with $f\geq m/3$ Byzantine validators. Divide the $m$ validators into three sets: $A$, $B$, and $C$ each with at least one validator and at most $f$ validators. Divide all the clients into two sets: $X$ and $Y$ each with at least one client. We consider the following three worlds and explain the worlds from the view of $A$, $B$, $C$, $X$ and $Y$.

\noindent {\bf World 1:} In World 1 validators in $A$ and $B$ start with the value 1. Validators in $C$ are Byzantine but pretend to be honest with initial value 0. Since $C$ has at most $f$ participants, the clients in $X$ must eventually commit a value by honest termination. For validity to hold, all the clients in $X$ will output 1. %From the perspective of $A$, $B$ and $X$, they cannot distinguish between a crashed (or Byzantine) $C$ vs. an honest $C$ whose messages are delayed.

\noindent{\bf World 2:} In World 2 validators in $B$ and $C$ start with the value 0. Validators in $A$ are Byzantine but pretend to be honest with initial value 1. Since $A$ has at most $f$ participants, the clients in $Y$ must eventually commit a value by honest termination. For validity to hold, all the clients in $Y$ will output 1.

\noindent{\bf World 3:} World 3 will be a hybrid world where the view of $X$ in this world will be indistinguishable to the view of $X$ in world 1 and the view of $Y$ in this world will be indistinguishable to the view of $Y$ in world 2. $A$ will start with value 1 and $C$ will start with value 0. The adversary will use its Byzantine power to corrupt $B$ to perform a split-brain attack and make $X$ and $Y$ each believe that they are in their respective worlds. $B$ will equivocate but act honestly as if its starting value is 1 when communicating with $X$ and as if its 0 when communicating with $Y$. Then by an indistinguishability argument, $X$ will commit 1 and $Y$ will commit 0. This violates the agreement property.

\hfill

\noindent \textit{If}: Assume $m>3f$, now we solve the problem of ABC client consensus in passive mode. The protocol is simple: the validators just send their values to all clients; and the client commits a value if it receives the same value from at least $2f+1$ validators. It is easy to check that this protocol satisfies agreement, validity and honest termination; Moreover, there is no communication among the validators.
\end{proof}

\section{Proof of Theorem~\ref{thm:active}}
\label{app:proof2}

\begin{proof}
Since in our model, the distributed protocols may or may not use PKI, we prove the strongest results: for the negative results (i.e., ``only if'' parts), we assume PKI is used; and for the positive results (i.e., ``if'' parts), we avoid using PKI.
\hfill

\noindent (1) Client consensus:

\noindent \textit{Only if}: %\kartik{Is this proof exactly the same as: \url{https://decentralizedthoughts.github.io/2019-06-25-on-the-impossibility-of-byzantine-agreement-for-n-equals-3f-in-partial-synchrony/}} \xw{Yes, just additionally take care of the clients.} 
Seeking a contradiction, let us assume there is a protocol that claims to solve client consensus with $f\geq m/3$ Byzantine validators. Divide the $m$ validators into three sets: $A$, $B$, and $C$ each with at least one validator and at most $f$ validators. Divide all the clients into two sets: $X$ and $Y$ each with at least one client. We consider the following three worlds and explain the worlds from the view of $A$, $B$, $C$, $X$ and $Y$. In all three worlds, we will assume that all messages between $A \longleftrightarrow B$ and $B\longleftrightarrow C$ arrive immediately. See Fig.~\ref{fig:converse1}.

\begin{figure*}
    \centering
    \includegraphics[width=0.85\textwidth]{figures/thm2_new.pdf}
    \caption{Different worlds in the proof of Theorem~\ref{thm:active}.}
    \label{fig:converse1}
\end{figure*}
%\peiyao{Do we have to crash clients $X$ and $Y$? Can we only consider $X$ in world 1 and $Y$ in world 2 (like lemma 3.4)?}

\noindent {\bf World 1:} In World 1 validators in $A$ and $B$ start with the value 1. Validators in $C$ and clients in $Y$ have crashed. Since $C$ has at most $f$ participants, the clients in $X$ must eventually commit a value by termination. For validity to hold, all the clients in $X$ will output 1. From the perspective of $A$, $B$ and $X$, they cannot distinguish between a crashed (or Byzantine) $C$ vs. an honest $C$ whose messages are delayed.

\noindent{\bf World 2:} World 2 will be a world similar to world 1 where the roles of $A$ and $C$ and the roles of $X$ and $Y$ are interchanged. The validators in $B$ and $C$ start with the value 0. Validators in $A$ and clients in $X$ have crashed. So all the clients in $Y$ will output 0 by termination and validity. Again, from the perspective of $B$, $C$ and $Y$, they cannot distinguish between a crashed $A$ vs. an honest $A$ whose messages are delayed. 

\noindent{\bf World 3:} World 3 will be a hybrid world where the view of $A$ and $X$ in this world will be indistinguishable to the view of $A$ and $X$ in world 1 and the view of $C$ and $Y$ in this world will be indistinguishable to the view of $C$ and $Y$ in world 2. $A$ will start with value 1 and $C$ will start with value 0. The adversary will use its Byzantine power to corrupt $B$ to perform a split-brain attack and make $A$ (or $X$) and $C$ (or $Y$) each believe that they are in their respective worlds. $B$ will equivocate and act as if its starting value is 1 when communicating with $A$ and $X$ and as if its 0 when communicating with $C$ and $Y$. If the adversary delays messages between $A \longleftrightarrow C$, $A \longrightarrow Y$ and $C \longrightarrow X$ for longer than the time it takes for $X$ and $Y$ to decide in their respective worlds, then by an indistinguishability argument, $X$ will commit to 1 and $Y$ will commit to 0. This violates the agreement property.

\hfill

\noindent \textit{If}: Assume $m>3f$, now we solve the problem of client consensus in active mode. The validators run any partial synchronous consensus protocol and send the committed value to the clients. The client commits a value if it receives the same value from at least $2f+1$ validators. %Since the network graph is $f+1$-connected, the subgraph induced by honest validators must be connected given the existence of at most $f$ Byzantine faults. So, as long as honest validators gossip all the messages, the point-to-point communication between any two honest validators will still be delivered eventually.
It is easy to check that this protocol satisfies agreement, validity and termination.

\hfill

\noindent (2) ABC client consensus: 

\noindent \textit{Only if}: Same as the proof for client consensus as above. Note that in world 1\&2 honest validators start with the same value, hence honest termination suffices for the proof.

\hfill

\noindent \textit{If}: Same as the algorithm that solves ABC client consensus in passive mode (in the proof of Theorem~\ref{thm:passive}).
\end{proof}

==> app_pseudo.tex <==
\section{Pseudocode of \tblite}
\label{app:tblite}

\input{tblite-protocol}


==> contract.tex <==


\begin{listing}[!ht]
\begin{minted}
[
%linenos,
highlightlines={5-6},
escapeinside=||
]{rust}
fn execute(contractInfo, |\colorbox{LightCyan}{executeMsg}|) {
    let funcName = executeMsg.funcName;
    let param = executeMsg.param;
    
    assert_eq!(contractInfo.sender, addressOfTB); 
    let TBInfo = executeMsg.TBInfo;
    
    match executeMsg {
        funcA -> funcA(|\colorbox{LightCyan}{TBInfo}|, param),
        funcB -> funcB(|\colorbox{LightCyan}{TBInfo}|, param),
        ...
    }
}
// definition of funcA, funcB...
\end{minted}
\caption{Handler of \appx contract with \tb proxy}
\label{listing:execute-tb}
\end{listing}


    



==> contract_execute.tex <==
\begin{listing}[!ht]
\begin{minted}
[
%linenos
]{rust}
fn execute(contractInfo, executeMsg) {
    let funcName = executeMsg.funcName;
    let param = executeMsg.param;
    match executeMsg {
        funcA -> funcA(contractInfo, param),
        funcB -> funcB(contractInfo, param),
        ...
    }
}
// definition of funcA, funcB...
\end{minted}
\caption{Entry point of CosmWasm contract}
\label{listing:execute}
\end{listing}


==> contract_sbs.tex <==
\begin{figure}[!h]
%  \vspace{-0.6cm}
 \begin{minipage}{0.5\textwidth}
  \centering
  \begin{minted}
[
linenos,
numbersep=-10pt,
frame=single,
fontsize=\scriptsize,
]{rust}
    fn execute(info, executeMsg) {
        let funcName = executeMsg.funcName;
        let param = executeMsg.param;
        
        
        
        
        
        match executeMsg {
            funcA -> funcA(info, param),
            funcB -> funcB(info, param),
            ...
        }
    }
    // definition of funcA, funcB...
\end{minted}
 \end{minipage}
 \begin{minipage}{0.5\textwidth}
  \centering
  \begin{minted}
[
fontsize=\scriptsize,
frame=single,
highlightlines={5-6},
escapeinside=||
]{rust}
fn execute(info, |\colorbox{LightCyan}{executeMsg}|) {
    let funcName = executeMsg.funcName;
    let param = executeMsg.param;
    
    assert_eq!(info.sender, addressOfTB); 
    let TBInfo = executeMsg.TBInfo;
    
    match executeMsg {
        funcA -> funcA(|\colorbox{LightCyan}{TBInfo}|, param),
        funcB -> funcB(|\colorbox{LightCyan}{TBInfo}|, param),
        ...
    }
}
// definition of funcA, funcB...
\end{minted}
 \end{minipage}
%   \vspace{-0.3cm}
 \caption{Left: Handler of CosmWasm contract. Right: Handler of \appx contract with \tb proxy. }
%  \vspace{-0.6cm}
 \label{fig:entry}
\end{figure}


==> contract_sbs_2.tex <==
\begin{figure}[!h]
 \begin{minipage}{0.5\textwidth}
  \centering
  \begin{minted}
[
breaklines,
frame=single,
]{rust}
fn execute(contractInfo, executeMsg) {
    let funcName = executeMsg.funcName;
    let param = executeMsg.param;
    match executeMsg {
        funcA -> funcA(contractInfo, param),
        funcB -> funcB(contractInfo, param),
        ...
    }
}
// definition of funcA, funcB...
\end{minted}
  \captionof{listing}{Sub caption}
 \end{minipage}
 \begin{minipage}{0.5\textwidth}
  \centering
  \begin{minted}
[
breaklines,
highlightlines={5-6},
frame=single,
escapeinside=||
]{rust}
fn execute(contractInfo, |\colorbox{LightCyan}{executeMsg}|) {
    let funcName = executeMsg.funcName;
    let param = executeMsg.param;
    
    assert_eq!(contractInfo.sender, addressOfTB); 
    let TBInfo = executeMsg.TBInfo;
    
    match executeMsg {
        funcA -> funcA(|\colorbox{LightCyan}{TBInfo}|, param),
        funcB -> funcB(|\colorbox{LightCyan}{TBInfo}|, param),
        ...
    }
}
// definition of funcA, funcB...
\end{minted}
  \captionof{listing}{Another sub caption}
 \end{minipage}
 \captionof{listing}{SomeCaption}
  \label{lst:representation_examples}
\end{figure}


==> imple_notes.tex <==
Consensus:
1. Constant storage
2. Constraint on IBC message:
- cannot self-deliver -> cannot trigger some event
- can only send IBC packet when return  
- Solution: message queue
Application:
- NameService: can only register for myself; does not allow proxy.
- if allow proxy, no change, just need to give TrustBoost the permission.

Evaluation:
f = 1,2,3?

1. Security
- Stress test: measure latency under malicious behavior, e.g., when the first a few leaders are malicious
- Network partition: start the relayers late.

2. Performance
- Measure latency: single chain vs. multi chain; scalable?
- Measure numbers of IBC messages: scalable?
- Measure gas fee (transaction fee + relayer fee): single chain vs. multi chain; scalable?
Say that pipelining/paralleling can increase throughput



==> meeting_notes.tex <==
1. Checkpointing. -- both original ideas (Nakamoto) and modern ones (Babylon). How is this related to the problem we are studying -- what does it solve we dont and vice versa
2. what are core bridge (IBC) activities and how Trustboost can improve their security. Definitely need to connect to Vitalik's post.

First shot at Q1. trustboost can replicate what checkpointing promises.
Second shot at Q1: checkpointing is L1 change while Trustboost is L2 change.

First shot at Q2. point out vitalik's example and how trustboost doesnt solve that. open question as to how to resolve it. need to think of a clever way of saying something about this open problem.
Second shot at Q2. look at practical bridge activities and point out one concrete use case that is easy to explain in English and can benefit from Trustboost.

==> old_proof.tex <==
% Comment out the lower bounds because these results are not complete.
\subsection{Lower bounds}

% \begin{theorem}
% \label{thm:consensus}
% Consensus can be achieved if and only if $m>3f$ and the network is $f+1$-connected.
% \end{theorem}

% \begin{theorem}
% \label{thm:abc}
% ABC can be achieved if and only if $m>3f$, but there is no requirement on network connectivity.
% \end{theorem}


Find minimum network connectivity and minimum communication cost in active mode.


\kartik{Can we use a variant of this proof here: \url{https://decentralizedthoughts.github.io/2019-08-16-byzantine-agreement-needs-quadratic-messages/}}

\xw{Ideas to extend this proof: 1) see what happens if there are two Byzantine validators; 2) one Byzantine validator + graphs that are not 2-connected (or 1-connected first).}

\xw{The conjecture that $f+1$-connected is necessary is wrong. Given a graph $G = (V,E)$, client consensus is possible even if $G$ is not connected: if there $\exists V_H \subseteq V$ s.t. $|V_H|\geq 3f+1$ and $G_H$ the subgraph induced by $V_H$ is $f+1$-connected, then we can let validators in $V_H$ run a consensus protocol and clients just ignore messages from $V	\setminus V_H$.

Note that here we assume nodes have complete knowledge of the communication graph $G$ as in~\cite{tseng2015fault}.

This is also an example where traditional consensus is impossible (as $G$ is not even connected) but client consensus can be achieved. 

Current conjecture on network connectivity: Given a graph $G = (V,E)$, if any subgraph $G'$ induced by a $V'$ with $V' \subseteq V$ and $|V'|\geq 3f+1$ is not $f+1$-connected, then client consensus is not possible.

Note that this example does not break our conjecture on quadratic communication cost yet. But it does invalidate the proof idea in \url{https://decentralizedthoughts.github.io/2019-08-16-byzantine-agreement-needs-quadratic-messages/} as client consensus can still be achieved even if some honest validators never receive any message.
}
\peiyao{I think the conjecture of $f+1$ connectivity is based on the assumption that  $n \ge 3f+1$ in the whole graph. If we know some subgraph has $n' > 3f+1$ then the connectivity requirement needs to be satisfied in the subgraph.}

\noindent {\bf Network connectivity.} A path $P$ in a graph $G = (V_G,E_G)$ is a finite sequence of edges which joins a sequence of distinct vertices. A graph $G$ is called connected if there is a path between every node pair in $G$; A graph $G$ is called $f+1$-connected if $G$ is connected after removing $f$ arbitrary nodes. A graph $G$ (with $|V_G| \geq 3f+1$) is called $f+1$-friendly if there is a connected component with at least $2f+1$ nodes after removing $f$ arbitrary nodes. Note that when $|V_G| = 3f+1$, $f+1$-connected is equivalent to $f+1$-friendly.

\xw{$\exists$ subgraph $G'=(V',E')$ s.t. $|V'|\geq 3f+1$ and $G'$ is $f+1$-connected implies $f+1$-friendly, but the other direction is not true (counterexample exists).}

\begin{theorem}
\label{thm:connectivity}
Suppose $m>3f$, consensus can be achieved if and only if G is $f+1$-friendly. \xw{different from traditional consensus}
\end{theorem}

\begin{lemma}
\label{lem:conn}
Suppose $m=3f+1$, consensus can be achieved if and only if G is $f+1$-connected. \xw{same as traditional consensus}
\end{lemma}

\begin{proof}

\hfill

\noindent \textit{If}: Assume $m=3f+1$ and the network is $f+1$-connected, now we solve the problem of consensus as defined in Definition~\ref{def:consensus}. The validators run any partial synchronous consensus protocol\kartik{need to separate the two consensus definitions here.} and send the quorum certificate to the clients when a value is committed. Since the network graph is $f+1$-connected, the subgraph induced by honest validators must be connected given the existence of at most $f$ Byzantine faults. So, as long as honest validators gossip all the messages, the point-to-point communication between any two honest validators will still be delivered eventually. Therefore, it is easy to check that this protocol satisfies agreement, validity and termination.

\hfill

\noindent \textit{Only if}: Seeking a contradiction, let us assume there is a protocol that solves consensus on a graph $G$ that is not $f+1$-connected. Then there exists a set of nodes $F$ such that $|F| = f$ and $G$ is not connected after removing $F$. Let there be $t>1$ connected components after removing $F$: $G_1 = (V_1, E_1), \cdots, G_t = (V_t, E_t)$ s.t. $|V_1|\geq \cdots \geq |V_t|\geq 1$. Divide all the clients into two sets: $X$ and $Y$ each with at least one honest client. The problem can be divided into two cases.


\noindent Case 1: $|V_1| \leq f$. We first construct the following $t+1$ worlds. See Figure~\ref{fig:converse3}.

\begin{figure}
    \centering
    \includegraphics[width=0.35\textwidth]{figures/converse3.png}
    \caption{Different worlds in the proof of Case 1 in Lemma~\ref{lem:conn}}
    \label{fig:converse3}
\end{figure}

\noindent {\bf World $1.i$ ($0\leq i \leq t$):} In world $1.i$, the validators in $\bigcup_{\ell=1}^i V_\ell$ start with value 0 and the validators in $\bigcup_{\ell=i+1}^t V_\ell$ start with value 1; validators in $F$ have crashed. By termination, in all $t+1$ worlds, clients in $X$ and $Y$ must eventually commit some value. By validity, the committed value must be 1 in world $1.0$ and 0 in world $1.t$. Then there must exist some integer $0\leq j\leq t-1$ such that the committed value is 1 in world $1.j$ and 0 in world $1.(j+1)$.

Then we define the following world:

    
\noindent {\bf World $2$:} World $2$ will be a hybrid world where the view of clients in $X$ in this world will be indistinguishable to their views in world $1.j$ and the view of clients in $Y$ in this world will be indistinguishable to their view in world $1.(j+1)$. In world $2$, the validators in $\bigcup_{\ell=1}^j V_\ell$ start with value 0 and the validators in $\bigcup_{\ell=j+2}^t V_\ell$ start with value 1. The adversary will use its Byzantine power to corrupt the validators in $V_{j+1}$ to perform a split-brain attack and make $X$ and $Y$ each believe that they are in their respective worlds. Note that $|V_{j+1}| \leq f$. The validators in $V_{j+1}$ will equivocate and act as if their starting values are 1 when communicating with $X$ and as if their starting values are 0 when communicating with $Y$. And since there is no communication among different components, the views of validators in other $t-1$ components will be indistinguishable to the views in worlds $1.j$ and $1.(j+1)$. Moreover, the adversary delays any message sent from $F$ until $X$ and $Y$ commit. Therefore, the view of $X$ in this world will be indistinguishable to the view of $X$ in world $1.j$ and the view of $Y$ in this world will be indistinguishable to the view of $Y$ to world $1.(j+1)$. Therefore, $X$ will commit 1 and $Y$ will commit 0. This violates the agreement property.
\peiyao{Shall $X$'s view be indistinguishable with world $1.j$ and $Y\sim 1.(j+1)$? The description here is inconsistent with Figure 3.} \xw{Fixed. Also simplified the proof a bit.}
\hfill

\noindent Case 2: $f+1 \leq |V_1| \leq 2f$. Let $\tilde V = \bigcup_{i=2}^t V_i$ and we have $|\tilde V| \leq f$. Let $|V_1| = f+k$ ($1\leq k \leq f$) and $|\tilde V| = f-k+1$. Divide $V_1$ into two sets $V_A$ and $V_B$ such that $|V_A| =f$ and $|V_B| = k$. We construct the following worlds. See Figure~\ref{fig:converse4}.

\begin{figure}
    \centering    \includegraphics[width=0.45\textwidth]{figures/converse4.png}
    \caption{Different worlds in the proof of Case 2 in Lemma~\ref{lem:conn}}
    \label{fig:converse4}
\end{figure}

\noindent {\bf World $1$:} In world 1, validators in $\tilde V$ and $V_B$ start with value $1$, and validators in $V_A$ start with value $0$. Validators in $F$ have crashed. By termination, clients in $X$ should commit some value, either 0 or 1.

\noindent {\bf World $2$:} In world 2, validators in $\tilde V$ and $V_B$ start with value $1$, and validators in $V_A$ start with value $0$ (all are the same as in world 1). Validators in $F$ start with value 1. Validators in $V_A$ are Byzantine but behave honestly. Since all honest validators start with value 1, clients in $X$ must commit 1 by validity. The adversary further delays messages sent from validators in $F$ until $X$ commits. Since the view of $X$ in world 2 is the same as in world 1, $X$ in both world 1 and world 2 will commit 1.

\noindent {\bf World $3$:} In world 3, validators in $\tilde V$ and $V_A$ start with value $0$, and validators in $V_B$ start with value $1$. Validators in $F$ have crashed. By termination, clients in $Y$ should commit some value, either 0 or 1.

\noindent {\bf World $4$:} In world 4, validators in $\tilde V$ and $V_A$ start with value $0$, and validators in $V_B$ start with value $1$ (all are the same as in world 3). Validators in $F$ start with value 0. Validators in $V_B$ are Byzantine but behave honestly. Since all honest validators start with value 0, clients in $Y$ must commit 0 by validity. The adversary further delays messages sent from validators in $F$ until $Y$ commits. Since the view of $Y$ in world 4 is the same as in world 3, $Y$ in both world 3 and world 4 will commit 0.

\noindent {\bf World $5$:} World $5$ will be a hybrid world where the view of clients in $X$ in this world will be indistinguishable to their views in world $2$ and the view of clients in $Y$ in this world will be indistinguishable to their view in world $4$. In world 5, validators in $V_A$ start with value $0$ and validators in $V_B$ start with value $1$. Validators in $F$ start with value 0. The adversary will use its Byzantine power to corrupt the validators in $\tilde V$ to perform a split-brain attack and make $X$ and $Y$ each believe that they are in their respective worlds. Note that $|\tilde V| \leq f$. The validators in $\tilde V$ will equivocate and act as if their starting values are 1 when communicating with $X$ and as if their starting values are 0 when communicating with $Y$. Moreover, the adversary delays any message sent from $F$ until $X$ and $Y$ commit. Hence, the views of validators in $V_A$ and $V_B$ will be indistinguishable to the views in worlds $2$ and $4$. Therefore, the view of $X$ in this world will be indistinguishable to the view of $X$ in world $2$ and the view of $Y$ in this world will be indistinguishable to the view of $Y$ to world $4$. Therefore, $X$ will commit 0 and $Y$ will commit 1. This violates the agreement property.

\end{proof}

\xw{To prove Theorem~\ref{thm:connectivity}, case 1 is the same. But for case 2, the proof does not go through when there are two components with size $\geq f+1$. Perhaps we need to change the definition of termination.} 

\noindent {\bf Communication cost.} We assume a fully connected validator network and only count messages among validators.

\begin{theorem}
Any consensus protocol that is resilient to $f$ Byzantine faults must have an execution where the honest validators send $\geq f/4$ messages among each other. \xw{can be easily strengthened to $f/2$}
\end{theorem}

\begin{proof}[Proof sketch]
We first find two neighboring worlds (say world 1 and world 2) where only one validator (say validator $a$) hold different initial value but all clients commit different values in the end. In world 1, $< f/2$ validators have received/sent messages from/to other validators, denoted as set $V_1$. In world 2, $< f/2$ validators have received/sent messages from/to other validators, denoted as set $V_2$. Then in world 3, the adversary corrupts $a \cup V_1 \cup V_2$ ($\leq f$ validates) to perform a split-brain attack that leads to an agreement violation.
\end{proof}


\iffalse
\begin{proof}[Proof of Theorem~\ref{thm:consensus}]
\hfill

\noindent \textit{If}: Assume $m>3f$ and the network is $f+1$-connected, now we solve the problem of consensus as defined in Definition~\ref{def:consensus}. The validators run any partial synchronous consensus protocol and send the quorum certificate to the clients when a value is committed. Since the network graph is $f+1$-connected, the subgraph induced by honest validators must be connected given the existence of at most $f$ Byzantine faults. So, as long as honest validators gossip all the messages, the point-to-point communication between any two honest validators will still be delivered eventually. Therefore, it is easy to check that this protocol satisfies agreement, validity and termination.

\noindent \textit{Only if}: We prove this part by showing the following two claims.
\begin{claim}
\label{claim:consensus1}
Consensus is impossible if $m \leq 3f$ (even when the validators are fully connected).
\end{claim}

\begin{proof}
\kartik{Is this proof exactly the same as: \url{https://decentralizedthoughts.github.io/2019-06-25-on-the-impossibility-of-byzantine-agreement-for-n-equals-3f-in-partial-synchrony/}} \xw{Yes, just additionally take care of the clients.}Seeking a contradiction, let us assume there is a protocol that claims to solve consensus with $f\geq m/3$ Byzantine validators. Divide the $m$ validators into three sets: $A$, $B$, and $C$ each with at least one validator and at most $f$ validators in each set. Divide all the clients into two sets: $X$ and $Y$ each with at least one client. We consider the following three worlds and explain the worlds from the view of $A$, $B$, $C$, $X$ and $Y$. In all three worlds, we will assume that all messages between $A \longleftrightarrow B$ and $B\longleftrightarrow C$ arrive immediately. See Figure~\ref{fig:converse1}.

\begin{figure}
    \centering
    \includegraphics[width=0.35\textwidth]{figures/converse1.png}
    \caption{Different worlds in the proof of Claim~\ref{claim:consensus1}}
    \label{fig:converse1}
\end{figure}

\noindent {\bf World 1:} In World 1 validators in $A$ and $B$ start with the value 1. Validators in $C$ and clients in $Y$ have crashed. Since $C$ has at most $f$ participants, the clients in $X$ must eventually commit a value by termination. For validity to hold, all the clients in $X$ will output 1. From the perspective of $A$, $B$ and $X$, they cannot distinguish between a crashed (or Byzantine) $C$ (or $Y$) vs. an honest $C$ (or $Y$) whose messages are delayed.

\noindent{\bf World 2:} World 2 will be a world similar to world 1 where the roles of $A$ and $C$ and the roles of $X$ and $Y$ are interchanged. The validators in $B$ and $C$ start with the value 0. Validators in $A$ and clients in $X$ have crashed. So all the clients in $Y$ \peiyao{$Y$?} \xw{yes.} will output 0 by termination and validity. Again, from the perspective of $B$, $C$ and $Y$, they cannot distinguish between a crashed $A$ (or $X$) vs. an honest $A$ (or $X$) whose messages are delayed. 

\noindent{\bf World 3:} World 3 will be a hybrid world where the view of $A$ and $X$ in this world will be indistinguishable to the view of $A$ and $X$ in world 1 and the view of $C$ and $Y$ in this world will be indistinguishable to the view of $C$ and $Y$ in world 2. $A$ will start with value 1 and $C$ will start with value 0. The adversary will use its Byzantine power to corrupt $B$ to perform a split-brain attack and make $A$ (or $X$) and $C$ (or $Y$) each believe that they are in their respective worlds. $B$ will equivocate and act as if its starting value is 1 when communicating with $A$ and $X$ and as if its 0 when communicating with $C$ and $Y$. If the adversary delays messages between $A \longleftrightarrow C$, $A \longrightarrow Y$, $C \longrightarrow X$ and $X \longleftrightarrow Y$ for longer than the time it takes for $X$ and $Y$ to decide in their respective worlds, then by an indistinguishability argument, $X$ will commit to 1 and $Y$ will commit to 0. This violates the agreement property.
\end{proof}

\begin{claim}
\label{claim:consensus2}
Consensus is impossible if there is no edge in the validator network (even when there is only one Byzantine validator).
\xw{Needs to strengthen this claim to a $f+1$-connected network. Still working on it.}
\end{claim}

\begin{proof}
Seeking a contradiction, let us assume there is a protocol that claims to solve consensus when there is no edge in the validator network. Divide all the clients into two sets: $X$ and $Y$ each with at least one client. We first construct the following $m+1$ worlds. See Figure~\ref{fig:converse2}.

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/converse2.png}
    \caption{Different worlds in the proof of Claim~\ref{claim:consensus2}}
    \label{fig:converse2}
\end{figure}

\noindent {\bf World $1.i$ ($0\leq i \leq m$):} In world $1.i$, the first $i$ validators start with value 0 and the rest $m-i$ validators start with value 1. Clients in $Y$ have crashed. By termination, in all $m$ worlds, clients in $X$ must eventually commit some value. By validity, the committed value must be 1 in world $1.0$ and 0 in world $1.m$.\peiyao{why? in world 1.1 only the first validator starts with value 0.}\xw{Fixed.} Then there must exist some integer $0\leq j\leq m-1$ such that the committed value is 1 in world $1.j$ and 0 in world $1.(j+1)$.

Then we define the following two worlds:

\noindent {\bf World $2.j$:} In world $2.j$, the first $j$ validators start with value 0 and the rest $m-j$ validators start with value 1. Clients in $X$ have crashed. By termination, clients in $Y$ must eventually commit some value. 

\noindent {\bf World $2.(j+1)$:} In world $2.(j+1)$, the first $j+1$ validators start with value 0 and the rest $m-j-1$ validators start with value 1. Clients in $X$ have crashed. By termination, clients in $Y$ must eventually commit some value. 

Next, the problem can be divided into three cases:

\noindent \textit{Case 1.} Clients in $Y$ commit 0 in world $2.j$. Then we consider the following world.
    
\noindent {\bf World $3$:} In world $3$, the first $j$ validators start with value 0 and the rest $m-j$ validators start with value 1. The messages between $X$ and $Y$ are delayed by the adversary. However, the view of $X$ in this world will be indistinguishable to the view of $X$ in world $1.j$ and the view of $Y$ in this world will be indistinguishable to the view of $Y$ to world $2.j$. Therefore, $X$ will commit 1 and $Y$ will commit 0. This violates the agreement property.

\noindent \textit{Case 2.} Clients in $Y$ commit 1 in world $2.(j+1)$. This case can be contracted in the same way as case 1.

\noindent \textit{Case 3.} Clients in $Y$ commit 1 in world $2.j$ and clients in $Y$ commit 0 in world $2.(j+1)$. Then we consider the following world.
    
\noindent {\bf World $3'$:} World $3'$ will be a hybrid world where the view of the first $j$ validators and $X$ in this world will be indistinguishable to their views in world $1.(j+1)$ and the view of the last $m-j-1$ validators and $Y$ in this world will be indistinguishable to their view in world $2.j$. In world $3'$, the first $j$ validators start with value 0 and the last $m-j-1$ validators start with value 1. The adversary will use its Byzantine power to corrupt the $j$-th validator to perform a split-brain attack and make $X$ and $Y$ each believe that they are in their respective worlds. The $j$-th validator will equivocate and act as if its starting value is 0 when communicating with $X$ and as if its 1 when communicating with $Y$.
The messages between $X$ and $Y$ are delayed by the adversary. And since there is no communication among the validators, their views will be indistinguishable to the views in their respective worlds. Moreover, the view of $X$ in this world will be indistinguishable to the view of $X$ in world $1.(j+1)$ and the view of $Y$ in this world will be indistinguishable to the view of $Y$ to world $2.j$. Therefore, $X$ will commit 0 and $Y$ will commit 1. This violates the agreement property.


\end{proof}

Combining the two claims above, we can conclude the proof.

\end{proof}


\begin{proof}[Proof of Theorem~\ref{thm:abc}]
\hfill

\noindent \textit{If}: Assume $m>3f$, now we solve the problem of consensus as defined in Definition~\ref{def:abc}. The protocol is simple: the validators just sign their values and send the signed values to all clients; and the client commits a value if it receives at least $2f+1$ different signatures for the same value (which form a quorum certificate for the committed value); further, a client will forward the certificate to all other clients when committing a value. It is easy to check that this protocol satisfies agreement, validity and honest termination, moreover, there is no communication among the validators.

\hfill

\noindent \textit{Only if}: The proof of this part is exactly the same as the proof for the condition $m>3f$ in Theorem~\ref{thm:consensus} (Claim~\ref{claim:consensus1}).

\begin{remark}
\label{rem:clients}
We assume the clients can communicate with each other. This assumption is needed in ABC. Otherwise, it is possible that only the adversary collects a certificate ($2f+1$ signatures) for some value and it can send it to only one honest client. Then only that honest client commits the value but others don't, which violates agreement. However, this assumption may not be needed in consensus and our protocol (\tbnosp). The clients do not need to communicate with each other if the protocol guarantees that: if the adversary obtains a certificate for some value, then honest validators will obtain certificates for the same value eventually. 
\end{remark}

\begin{proof}[Proof of Theorem~\ref{thm:lower_bound}]

\hfill

\xw{working on it.}
\end{proof}

\end{proof}

\fi

==> old_protocol.tex <==
\section{The \tb Protocol}
\label{sec:protocol}

\subsection{Blockchains as Validators}

In \tbnosp, each of the $m$ validators is instantiated as a programmable blockchains, through smart contracts deployed on top of a public verifiable ledger consensus protocol. The $i$-th blockchain ($1\leq i \leq m$) is run by a permissioned committee $C_i$ with $|C_i| = n_i$ of which at most $f_i$ nodes are Byzantine. We can see that each blockchain in \tb behaves the same as as a single validating node: the quorum certificates will work as the signatures; a blockchain with honest super-majority ($n_i > 3f_i$) will behave in the same way as an honest validator (i.e., no equivocation), otherwise it may behave arbitrarily (Byzantine). In addition, the communications between the blockchains are made possible by a primitive called inter-blockchain communication (IBC), a bidirectional ledger-to-ledger links~\cite{goes2020interblockchain}.

\subsection{Primitives}
In this section, we introduce several primitives used in the protocol.
%\xw{Needs to describe the protocol as smart contracts and describe IBC as a primitive.}

\myparagraph{Local consensus protocol.} $\plocal_k$ is a public verifiable ledger consensus protocol run by nodes in committee $C_k$, that is, any light client can check whether a message $msg$ is committed on the ledger. $\plocal_k$ can be instantiated by a black-box partial synchronous protocol, with following three basic components.
    \begin{itemize}
        \item[-] {\bf Signed message $\signed{msg}_i$}: traffic of the protocol message passes around the network in messages,  represents a message signed by node $i$ in committee $C_k$.
        \item[-] {\bf Reliable multicast }$\lmult_i(msg, j)$:  Node $i$ broadcasts a signed message $\signed{msg}_i$ to node $j$.
        \item[-] {\bf Reliable delivery }$\lrcv_j(\signed{msg}_i)$: When receiving a signed message $\signed{msg}_i$, node $j$ verifies the signature using $i$'s public key.
    \end{itemize}

\myparagraph{Inter-blockchain communication (IBC)} $IBC(msg, dst)$ is a routing protocol run by {\em relayers} that allows independent blockchains communicate with each other. Relayers are a set of independent rational nodes that follow IBC protocols by incentives. IBC is analogous to that of reliable broadcast, it takes the message and destination from inputs and realizes a reliable, in-order message stream.


\myparagraph{Global consensus protocol.} $\pglobal$ is a public verifiable ledger consensus protocol run by committees through smart contracts to regularly issue checkpoints on the $m$ local blockchains. $\pglobal$ can be instantiated by a black-box partial synchronous protocol in a similar way to $\plocal_i$, by replacing basic components accordingly. Besides, $\pglobal$ invokes $\plocal$ in each step.
    \begin{itemize}
        \item[-] {\bf Certified message} $(msg, \cert_i(msg))$: the message among blockchains contains the message and a certificate generated by committee $C_i$.
        \item[-] {\bf IBC }$\gmult_i(msg, j)$:  Committee $C_i$ sends a certified message $(msg, \cert_i(msg))$ to committee $C_j$ via IBC protocol (details are in Algorithm~\ref{alg:gmult}).
       \item[-] {\bf Global delivery }$\grcv_j(msg, \cert_i(msg))$: On receiving a certified message, committee $C_j$ validates the certificate and calls $\plocal_j$ to agree on the certified message $msg$.
    \end{itemize}



 
    
    
    
    




\subsection{\tb}
Suppose $n = n_1 = n_2 = \cdots n_m$, each node is assigned a unique id within the committee numbered from $1$ to $n$.

\begin{algorithm}[H]
\caption{$\gmult_i(msg, j)$}
\label{alg:gmult}
\begin{algorithmic}[1]
\If{$msg$ is not committed locally}
\State invoke $\plocal_i(msg)$, wait until $msg$ is committed with $ \cert_i(msg)$
\EndIf
\State Relayers multicast $(msg,\cert_i(msg))$ to committee $C_j$.
    %\For{$ k = 1, 2, \cdots, n$} 
    %\State node $k$ in committee $C_i$ sends $(msg,\cert_i(msg))$ to node $k$ in committee $C_j$. 
    %\EndFor
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[H]
\caption{$\grcv_j(msg, \cert_i(msg))$}
\label{alg:grcv}
\begin{algorithmic}[1]
    \For{any node $k$ in committee $C_j$} 
        \Upon{a valid message $(msg,\cert_i(msg))$}
        %\If{$msg$ is from node $k$ in committee $C_i$}
          %  \State broadcast $(msg,\cert_i(msg))$ to all nodes in committee $C_j$
       % \EndIf
        \If{$msg$ is the first valid message in current round}
            %\State $msg'\gets [msg, reply]$ \Comment{$reply$ is specified by $\pglobal$ protocol} %\xw{$\pglobal$? Do we need consensus on $msg$ so that honest nodes give the same $reply$?}
            \State invoke $\plocal_j(msg)$
        \EndIf
        \EndUpon
        \If{$msg$ is committed by $\plocal_j(msg)$}
            \State broadcast $\signed{reply}_k$ \Comment{$reply$ is generated
            by $\pglobal$} 
        \EndIf
        \Upon{$f_j + 1$ signed identical replies}
            \State $\cert_j(reply)\gets$ threshold signature of $f_j + 1$ replies
            \State commit $(reply, \cert_j(reply))$.
        \EndUpon
    \EndFor
\end{algorithmic}
\end{algorithm}

\subsection{\tblite}
\label{sec:lite}

Here we propose a light-weight protocol called \tblite that solves the problem of ABC ledger consensus as defined in Definition~\ref{def:abc_ledger}. In \tblitenosp, the transactions use the unspent transaction output (UTXO) model.

\begin{itemize}
    \item Each blockchain can be independent and no cross-chain communication is needed.
    \item Only requirement for ``honest'' blockchain: does not contain double-spend (transactions that share the same inputs).
    \item Confirmation: A transaction is confirmed if 1) it is committed in 2/3 of the blockchains and 2) all its inputs are outputs from confirmed transactions. Confirmation can be done by clients who can read all blockchains.
\end{itemize}

==> reviews.tex <==
FC 23
Review A:
I really liked the problem and the paper motivation; boosting collective security of interoperable systems (that may even have different settings/properties) is of great value. However, I am afraid that the paper cannot be published in its current state due to the following reasons:

- The solution is very customized to the Cosmos network (which has several disadvantages on its own and it is not an ideal solution for blockchain interoperability). I see it like a solution to avoid the centralized trusted hub problem of Cosmos rather than a generic (or general) trust booster or combiner of arbitrary blockchains. Also it works only with smart contract-enabled blockchains rather than any blockchain (e.g., UTXO-based ones).

- I found the model very strong and very specific to permissioned blockchains rather than permissionless blockchains where in my opinion, the trust and faulty behavior matters more. Permissioned are usually composed of accountable nodes deployed by big companies/entities, so trust and faulty behavior is more controlled.

Also, and as outlined in 2.1, assuming all participants are connected with authenticated channels, with a PKI for all validators, and have full connectivity among themselves, are very strong assumptions that are far from what we have in public permissionless blockchains.

- The related work is very brief and does not discuss all related concepts to the work, e.g., blockchain interoperability, hybrid consensus, etc.

- On page 7, it is mentioned that each participating blockchain is managed by a permissioned committee. Who selects this committee? Are the members outsiders or a subset of the local blockchain miners?

- Is there a global blockchain that logs the agreed upon state of the local blockchains? or the state is derived from the states of the individual smart contracts deployed on the local blockchains?

- I do not see how the solution can be extended to support heterogeneous blockchains or anything other than Cosmos. What if these blockchains do not support the CCC protocol?

- Even for the TrustBoost Lite version, where it is mentioned that it works in the UTXO model, I was not able to see how then the BFT will run without smart contracts?

- The security of the protocols is discussed very briefly and informally. A more formal and detailed analysis is needed.

- Many details are missing and the discussion in many parts is rather a high level, which makes it hard to follow the paper and vet the design.

Overall, I still think the problem is interesting, but the presented solution does not match the impression that I got from the abstract and the introduction---these give the impression that a general solution is proposed, while it is not the case.


Review B:
- The construction does not work on the current cosmos ecosystem. The smart contracts proposed must be deployed through governance changes in the underlying protocols, which makes deployment impractical.
- This construction has already been explored in the IBC world [0] in terms of "recursive tendermint". The construction proposed is also in cosmos land, and is very similar, even drawing the same analogies. The novelty of the paper is still good, but this should definitely be cited! I'm not sure if the authors are aware of this.

Overall I enjoyed reading this paper and I think it would make a great addition to FC.

[0] https://github.com/cosmos/ibc/issues/547


Review C:
** Comparison with related work
The manuscript mentions several works that are related to the ideas presented in this paper. However, this part would need to be expanded in order to make clearer what is the concrete contribution of this work and/or tradeoffs with related works.

** Client consensus and ABC client consensus notions

Following with the previous point, it is unclear to me how novel are the notions of client consensus and ABC client consensus. The authors do mention that ABC client consensus is a somewhat relaxed notion from that in [28] without further explanation. Moreover, the description of these notions are rather high level. I believe that these notions need to be formally and thoroughly described in order to properly evaluate the "theoretical" results presented later in the paper. 

** TrustBoost 

I would have liked to see the insights on the technical challenges when designing TrustBoost. As presented now, it looks like a simple wrapper over well established building blocks such as consensus committees for the underlying blockchains as well as cross-chain communication protocols. In fact, the informal proof sketch for the security seem to show that TrustBoost is seamlessly secure if enough of the underlying consensus protocols are secure.

** Implementation

Perhaps, the most interesting part of the paper is the implementation of TrustBoost and the different engineering efforts that the authors have taken in order to make it work with available blockchain project such as Cosmos. Also, the evaluation, although short, it is interesting as it shows the scalability with the number of underlying blockchains. I would have liked to see a more elaborated descriptions of the attacks considered in the evaluation. Also, it would have been interesting to see the USD cost of the different operations in table 1, which are currently only shown in gas cost.



ConsensusDay 23
Review A:
Some definitions are not clear and hard to digest. For ABC client consensus, the honest termination definition, if honest validators start with different values they don’t need to terminate? Also, all termination properties are defined as “if messages are delivered quickly then terminates quickly”. Why not define termination under the standard partial synchronous assumption, i.e., eventually (after GST) the protocols terminate? The difference between client ledger consensus and ABC client ledger consensus is hard to digest from the definitions. It would be better if some examples could be provided.

There is little novelty at the protocol level, as the paper directly uses the existing IT-Hotstuff. An interesting future direction may be how to design a consensus that is suitable for smart contract implementation. It is also not clear if the problem can be solved with asynchronous protocols (which may provide better latency guarantees) assuming there is some on-chain randomness beacon that can be used.

There might still be room to improve the implementation of the protocol in terms of latency and gas cost, in future work.


Review B:
p1: it is said "a form of "consensus on top of consensus," a first in the literature." There were previous works that did things like that. To the best of my knowledge, Steward [A] was the first one.

[A] Yair Amir, Claudiu Danilov, Danny Dolev, Jonathan Kirsch, John Lane, Cristina Nita-Rotaru, Josh Olsen, David Zage. STEWARD: Scaling Byzantine Fault-Tolerant Replication to Wide Area Networks. IEEE Transactions on Dependable and Secure Computing, Volume 7 Number 1, pp. 80-93, 2010.

p3: I have several comments about the description of (ABC) client consensus problem:

you can remove "If messages are delivered quickly, the consensus protocol terminates quickly" from all Termination properties on the problem statements. First, because it is not termination (nor Liveness); second, because it precludes the use of blockchains that does not satisfy responsiveness (whose latency is not proportional to network latency)

client consensus is quite similar to a read from an atomic register emulation in which the underlying value is undetermined. If a client reads a value, all clients need to read the same. I'm not sure this formulation is better than the one you have.

in the case of ABC consensus and considering the register formulation, you can do better. For example, suppose you can differentiate the freshness of 0 and 1 (and this doesn't seem complicated when processes are blockchains). In that case, deterministically selecting the freshest value (0 or 1) is possible if a client receives more than 2f+1 of these. This might require more than 3f+1 servers, but the definition of the problem you are using is too simple to represent what can be done in practice accurately. So, maybe (just maybe) some of the conditions in section 3 are unnecessary.

The implementation and evaluation are pretty straightforward, but the originality of the approach makes them a substantial contribution of the work. I particularly liked the discussion about the limitations of implementing consensus on top of the smart contracts framework.

The discussion section is also very interesting and can bring a lot of interest to the audience.

Overall, I liked the paper and think it should appear on the consensus day program.

==> tables.tex <==
\begin{table}[]
    \centering
    \vspace{-0.6cm}
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        m & 1 & 4 & 7 & 10 \\
        \hline
        \hline
        \# IBC messages & 0 & 102 & 348 & 738\\
        \hline
        Gas usage & 202.1K & 73.7M & 260.5M & 585.6M \\
        \hline
        Latency & 2.5s &  67.2s & 105.0s & 138.2s \\
        \hline
    \end{tabular}
    \caption{Performance of \tb with different number of chains.}
    \vspace{-1cm}
    \label{tab:perf}
\end{table}


\begin{table}[]
    \centering
    \vspace{-0.5cm}
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        Attacks & I & II & III & IV \\
        \hline
        \hline
        Latency &  & & 66.8s & 66.0s \\
        \hline
    \end{tabular}
    \caption{Performance of \tb under different attacks.}
    \vspace{-1cm}
    \label{tab:sec}
\end{table}
